PALP: Prompt Aligned Personalization of Text-to-Image Models

Content creators often aim to create personalized images using personal subjects that go beyond the capabilities of conventional text-to-image models. Additionally, they may want the resulting image to encompass a specific location, style, ambiance, and more. Existing personalization methods may compromise personalization ability or the alignment to complex textual prompts. This trade-off can impede the fulfillment of user prompts and subject fidelity. We propose a new approach focusing on personalization methods for a \emph{single} prompt to address this issue. We term our approach prompt-aligned personalization. While this may seem restrictive, our method excels in improving text alignment, enabling the creation of images with complex and intricate prompts, which may pose a challenge for current techniques. In particular, our method keeps the personalized model aligned with a target prompt using an additional score distillation sampling term. We demonstrate the versatility of our method in multi- and single-shot settings and further show that it can compose multiple subjects or use inspiration from reference images, such as artworks. We compare our approach quantitatively and qualitatively with existing baselines and state-of-the-art techniques.

==> 3_method.tex <==
\section{Preliminaries}
\label{sec:personalization}

\paragraph{Generative Diffusion Models.} 
Diffusion models perform a backward diffusion process to generate an image. In this process, the diffusion model $G$ progressively denoises a source $x_T \sim \mathcal{N}(0,1)$ to produce a real sample $x_0$ from an underlying data distribution $p(X)$. At each timestep $t \in \{0,1,...,T\}$, the model predicts a noise $\hat{\epsilon} = G\left(x_t, t, y; \theta\right)$ conditioned on a prompt $y$ and timestep $t$. The generative model is trained by maximizing the evidence lower bound (ELBO) using a denoising score matching objective~\cite{DDPM}:

\begin{equation}
\label{eq:diff}
\mathcal{L}(\textbf{x},y) = \mathbb{E}_{t \sim [0,T], \epsilon \sim \mathcal{N}(0,1)} \left[\lVert G\left(x_t, t, y; \theta\right) - \epsilon \rVert_{2}^{2} \right].
\end{equation}

Here, $x_t = \sqrt{\bar{\alpha}_{t}} \textbf{x} + \sqrt{1-\bar{\alpha}_{t}}\epsilon$, and $\textbf{x}$ is a sample from the real-data distribution $p(X)$. Throughout this section, we will write $G_{\theta}(x_t, y) = G\left(x_t, t, y; \theta\right)$.

\paragraph{Personalization.} Personalization methods fine-tune the diffusion model $G$ for a new target subject $S$, by optimizing~\cref{eq:diff} on a small set of images representing $S$. Textual-Inversion~\cite{TI} optimizes new word embeddings to represent the new subject. This is done by pairing a generic prompt with the placeholder $[V]$, e.g., ``A photo of [V]'', where $[V]$ is mapped to the newly-added word embedding. DreamBooth~\cite{DB} calibrates existing word-embeddings to represent the personal subject $S$. This can be done by adjusting the model weights, or using recent more efficient methods that employ a Low-Rank Adaptation (LoRA)~\cite{LORA} on a smaller subset of weights~\cite{CustomDiffusion, simoLoRA2023, KeyLocked}.

\section{Prompt Alignment Method}
\label{sec:method}

\input{figures/method_overview/fig}
\subsection{Overview}
Our primary objective is to teach $G$ to generate images related to a new subject $S$. However, unlike previous methods, we strongly emphasize achieving optimal results for a \emph{single textual prompt}, denoted by $y$. For instance, consider a scenario where the subject of interest is one's cat, and the prompt is $y = \text{``A sketch of [my cat] in Paris.''}$ In this case, we aim to generate an image that faithfully represents the cat while incorporating all prompt elements, including the sketchiness and the Parisian context. 

The key idea is to optimize two objectives: personalization and prompt alignment. For the first part, i.e., personalization, we fine-tune $G$ to reconstruct $S$ from noisy samples. One option for improving prompt alignment would be using our target prompt $y$ as a condition when tuning $G$ on $S$. However, this results in sub-optimal outcome since we have no images depicting $y$ (e.g., we have no sketch images of our cat, nor photos of it in Paris). Instead, we push $G$'s noise prediction towards the target prompt $y$. In particular, we steer $G$'s estimation of $S$ towards the distribution density $p(x|y)$ using score-sampling methods (See~\cref{fig:overview}). By employing both objectives simultaneously, we achieve two things: (1) the ability to generate the target subject $S$ via the backward-diffusion process (personalization) while (2) ensuring the noise-predictions are aligned with text $y$. We next explain our method in detail.

\subsection{Personalization}
We follow previous methods~\cite{TI, DB, CustomDiffusion, KeyLocked}, and fine-tune $G$ on a small set of images representing $S$, which can be as small as a single photo. We update $G$'s weights using LoRA method~\cite{LORA}, where we only update a subset of the network's weights $\theta_{\text{LoRA}} \subseteq \theta $, namely, the self- and cross- attention layers. Furthermore, we optimize a new word embedding $[V]$ to represent $S$.






\subsection{Prompt-Aligned Score Sampling}

Long fine-tuning on a small image set could cause the model to overfit. In this case, the diffusion model predictions always steer the backward denoising process towards one of the training images, regardless of any conditional prompt. Indeed, we observed that overfitted models could estimate the inputs from noisy samples, even in a single denoising step (see supplemental material).

Our key idea is to encourage the model's denoising prediction towards the target prompt. Alternatively, we push the model's estimation of the real-sample, denoted by $\hat{x}_0$, to be aligned with the prompt $y$. The real-sample estimation $\hat{x}_0$ is derived from the model's noise prediction via:
\begin{equation}
\label{eq:x0_hat}
   \hat{x}_0  = \frac{x_t - \sqrt{1-\bar{\alpha}_{t}}G_{\theta}(x_t,y) }{ \sqrt{\bar{\alpha}_{t}} }.
\end{equation} 
In our example, where the target prompt is "A sketch of [V]," we push the model prediction toward a sketch and prevent overfitting a specific image background. Together with the personalization loss, this will encourage the model to focus on capturing [V]'s identifying features rather than reconstructing the background and other distracting features. 

To achieve the latter, we use Score Distillation Sampling (SDS) techniques~\cite{SDS}. In particular, given a clean target prompt $y^c$, that doesn't contain the placeholder "[V]". Then we use score sampling to optimize the loss:
\begin{equation}
\label{eq:palp_loss}
\mathcal{L}(\hat{x}_0,y^c),
\end{equation}
from~\cref{eq:diff}. Note, we use the pre-trained network weights to evaluate~\cref{eq:palp_loss}, and omit all learned placeholder (e.g., $[V]$). Therefore, this ensures that by minimizing the loss, we will stay aligned with the textual prompt $y$ since the pre-trained model possesses all knowledge about the prompt elements.

Poole et al.~\cite{SDS} found an elegant and efficient approximation of the score function using:
\begin{equation}
\label{eq:sds}
\nabla \mathcal{L}_{SDS}(\textbf{x}) =  \Tilde{w}(t) \left(G^{\alpha}\left(x_t, t, y^c; \theta\right) - \epsilon\right) \frac{\partial \textbf{x}}{\partial \phi},
\end{equation}
where $\phi$ are the weights controlling the appearance of $\textbf{x}$, and $\Tilde{w}(t)$ is a weighting function. Here $G^{\alpha}$ denotes the classifier-free guidance prediction, which is an extrapolation of the conditional and unconditioned ($y=\emptyset$) noise prediction. The scalar $\alpha \in \mathbb{R}^+$ controls the extrapolation via:
\begin{equation}
\label{eq:cfg}
    G^{\alpha}\left(x_t, t, y^c; \theta\right) =  (1-\alpha) \cdot G_{\theta}\left(x_t, \emptyset \right) + \alpha \cdot G_{\theta}\left(x_t, y^c \right).
\end{equation}

In our case, $\textbf{x} = \hat{x}_{0}$, and it is derived from $G$'s noise prediction as per~\cref{eq:x0_hat} . Therefore, the appearance of $\hat{x}_0$ is directly controlled by the LoRA weights and $[V]$. 


\subsection{Avoiding Over-saturation and Mode Collapse}
\label{sec:PALP_score}
Guidance by SDS produces less diverse and over-saturated results. Alternative implementations like~\cite{ProlificDreamer, NFSD} improved diversity, but the overall personalization is still affected (see supplemental for qualitative samples). We argue that the reason behind this is that the loss in~\cref{eq:sds} pushes the prediction $\hat{x}_0$ towards the center of distribution of $p(x|y^c)$, and since the clean target prompt $y^c$ contains only the subject class, i.e., ``A sketch of a cat'', then as a result, the loss will encourage $\hat{x}_0$ towards the center of distribution of a general cat, not our one. 

Instead, we found the Delta Denoising Score (DDS)~\cite{DDS} variant to work better. In particular, we use the residual direction between the personalized model's prediction $G^\beta_{\theta_{LoRA}} (\hat{x}_t, y_{P})$, and the pre-trained one $G^\alpha_{\theta}(\hat{x}_t, y^c)$, where $\alpha$ and $\beta$ are their guidance scales, respectively. Here $y_P$ is the personalization prompt, i.e., "A photo of [V]," and $y_c$ is a clean prompt, e.g., "A sketch of a cat."  The score can then be estimated by: 
\begin{equation}
\label{eq:palp_grad}
\nabla \mathcal{L}_{PALP} = \Tilde{w}(t) ( G^\alpha_{\theta}(\hat{x}_t, y^c) - G^\beta_{\theta_{LoRA}} (\hat{x}_t, y_{P})) \frac{\partial \hat{x}_0}{\partial \theta_{\text{LoRA}}},
\end{equation} which perturbs the denoising prediction towards the target prompt (see right part of~\cref{fig:overview}). Our experiments found imbalanced guidance scales, i.e., $\alpha > \beta$, to perform better. We have also considered two variant implementations: (1) in the first, we use the same noise for the two branches, i.e., the text-alignment and personalization branches, and (2) we use two i.i.d noise samples for the branches. Using the same noise achieves better text alignment than the latter variant.

\paragraph{On the Computational Complexity of PALP: } the gradient in~\cref{eq:palp_grad}, is proportional to the personalization gradient with the scaling:
\begin{equation}
     \frac{\partial \hat{x}_0}{\partial \theta_{\text{LoRA}}} \propto  - \frac{\sqrt{1-\bar{\alpha}_{t}}}{ \sqrt{\bar{\alpha}_{t}} } \nabla G_{\theta_{LoRA}}(x_t,y_P).
\end{equation} 
and since the gradient $\nabla G_{\theta_{LoRA}}(x_t,y_P)$ is also calculated as part of the derivative of~\cref{eq:diff}, then, we do not need to back-propagate through the text-to-image model through the prompt-alignment branch. This may be useful to use guidance from bigger models to boost smaller model's personalization performance. Finally, we also note that the scaling term is very high for large $t$-values. Re-scaling the gradient back by $  \sqrt{\bar{\alpha}_{t}} / \sqrt{1-\bar{\alpha}_{t}} $ ensures uniform gradient update across all timesteps and improves numerical stability.

 

==> 4_results.tex <==
\section{Results}

\input{figures/qualitative_comparison_multi/fig}

\paragraph{Experimental setup:} We use StableDiffusion (SD)-v1.4~\cite{LDM} for ablation and comparison purposes, as many official implementations of state-of-the-art methods are available in SD-v1.4. We further validate our method with larger text-to-image models (please refer to supplemental materials for further details). Complete experimental configuration, including learning rate, number of steps, and batch size, appear in the supplemental material. 

\paragraph{Evaluation metric: } for evaluation, we follow previous works~\cite{DB, TI} and use CLIP-score~\cite{CLIP} to measure alignment with the target (clean) prompt $y^c_t$ (i.e., does not have the placeholder [V]). For subject preservation, we also use CLIP feature similarity between the input and generated images with the target prompt. We use VIT-B32~\cite{VIT} trained by OpenAI on their proprietary data for both metrics. This ensures that the underlying CLIP used by SD-v1.4 differs from the one used for evaluation, which could compromise the validity of the reported metric.

\paragraph{Dataset: } for multi-shot setting, we use data collected by previous methods~\cite{TI, CustomDiffusion}, with different subjects like animals, toys, personal items, and buildings. For those subjects, checkpoints of previous methods exist, allowing a fair comparison. 

\subsection{Ablation studies}
\input{figures/ablation/fig}
For ablation, we start with TI~\cite{TI} and DB~\cite{DB} as our baseline personalization method and gradually add different components contributing to our final method. Full experimental details appear in the supplemental materials. 

\emph{\textbf{Early stopping: }} We begin by considering early stopping as a way to control the text-alignment. The lower the number of iterations, the less likely we are to hurt the model's prior knowledge. However, this comes at the cost of subject fidelity, evident from ~\cref{fig:ablation}. The longer we tune the model on the target subject, the more we risk overfitting the training set.

\emph{\textbf{Adding SDS guidance:}} improves text alignment, yet it severely harms the subject fidelity, and image diversity is substantially reduced (see supplemental materials). Alternative distillation sampling guidance~\cite{NFSD}  improves on top of SDS; however, since the distillation sampling guides the personalization optimization towards the center of distribution of the subject class, it still produces less favorable results.

 \emph{\textbf{Replacing SDS with PALP guidance:}}  improves text alignment by a considerable margin and maintains high fidelity to the subject $S$. We consider two variants: one where we use the same noise for personalization loss or sample a new one from the normal distribution. Interestingly, using the same noise helps with prompt alignment. Furthermore, scaling the score sampling equation~\cref{eq:palp_grad} by  $ \sqrt{\bar{\alpha}_{t}} / \sqrt{1-\bar{\alpha}_{t}}$ further enhances the performance. Further analysis and qualitative samples appear in the supplemental material.


\subsection{Comparison with Existing Methods}
\input{figures/quantative_table/quantiative_table}
\input{figures/user-study/table}
We compare our method against multi-shot methods, including CustomDiffusion~\cite{CustomDiffusion}, $P+$~\cite{PPLUS}, and NeTI~\cite{NeTI}. We further compare against TI~\cite{TI} and DB~\cite{DB} using our implementation, which should also highlight the gain we achieve by incorporating our framework with existing personalization methods. Our evaluation set contains ten different complex prompts that include at least four different elements, including style-change (e.g., "sketch of", "anime drawing of"), time or a place (e.g., "in Paris", "at night"), color palettes (e.g., "warm," "vintage"). We asked users to count the number of elements that appear in the image (text-alignment) and rate the similarity of the results to the input subject (personalization, see ~\cref{tab:multishot_quantitative_comp}).

Our method achieves the best text alignment while maintaining high image alignment. TI+DB achieves the best image alignment. However, the reason for this is because TI+DB is prone to over-fitting. Indeed, investigating each element in the prompt, we find that the TI+DB achieves the best alignment with the class prompt (e.g., "A  photo of a cat") while being significantly worse in the Style prompt (e.g., "A sketch"). Our method has a slightly worse image alignment since we expect appearance change for stylized prompts. We validate this hypothesis with a user study and find that our method achieves the best user preference in prompt alignment and personalization (see~\cref{tab:user_study}). Full details on the user study appear in the supplemental material.

\subsection{Applications}
\input{figures/qualitative_comparison_faces/fig}
\paragraph{Single-shot setting:} In a single-shot setting, we aim to personalize text-2-image models using a single image. This setting is helpful for cases where only a single image exists for our target subject (e.g., an old photo of a loved one). For this setting, we qualitatively compare our method with encoder-based methods, including IP-Adapter~\cite{IPAdapter}, ProFusion~\cite{ProFusion}, Face0~\cite{Face0}, and E4T~\cite{E4T}. We use portraits of two individuals and expect previous methods to generalize to our selected images since all methods are pre-trained on human faces. Note that E4T~\cite{E4T} and ProFusion~\cite{ProFusion} also perform test time optimization.

As seen from~\cref{fig:faces_qualitative}, our method is both prompt- and identity-aligned. Previous methods, on the other hand, struggle more with identity preservation. We note that optimization-based approaches~\cite{E4T, ProFusion} are more identity-preserving, but this comes at the cost of text alignment. Finally, our method achieves a higher success rate, where the quality of the result is independent of the chosen seed. 


\paragraph{Multi-concept Personalization: } Our method accommodates multi-subject personalization via simple modifications. Assume we want to compose two subjects, $S_1$ and $S_2$, in a specific scene depicted by a given prompt $y$. To do so, we first allocate two different placeholders, [V1] and [V2], to represent the target subjects $S_1$ and $S_2$, respectively. During training, we randomly sample an image from a set of images containing $S_1$ and $S_2$. We assign different personalization prompts $y_P$ for each subject, e.g., "A photo of [V1]" or "A painting inspired by [V2]", depending on the context. Then, we perform PALP while using the target prompt in mind, e.g., "A painting of [V1] inspired by [V2]". This allows composing different subjects into coherent scenes or using a single artwork as a reference for generating art-inspired images. Results appear in~\cref{fig:composition}; further details and results appear in the supplemental material. 

==> figures/teaser_v2/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/teaser_v2/TeaserV2.pdf}
    \caption{\ma{Need to rethink teaser}.}
    \label{fig:teaser_v2}
\end{figure}

==> sup_text.tex <==
\section{Introduction}
This document provides additional material not included in the main paper due to space constraints. In particular, we provide additional qualitative comparison for multi-shot setting, the results appear in~\cref{fig:multishot_qualitative_additional}. Moreover, a full qualitative comparison and un-curated results of the single-shot experiment appear in~\cref{fig:sup_faces_full_girl}, ~\cref{fig:sup_faces_full_guy}, and~\cref{fig:uncurated_single_shot}. For results obtained using a larger model, with improved text-encoder and bigger capacity, see~\cref{tab::LARGE_1} and~\cref{tab:LARGE_2}.

\input{sup_figures/Comp_additional/fig}

\section{Implementation Details}
All our experiments, except those conducted using a larger model, were conducted using TPU-v3, with a global batch size of 32. We use a learning rate of $\texttt{5e-5}$. For LoRA~\cite{LORA}, we use a rank $r=32$ and only modify the self-and cross-attention layers' projection matrices. For most experiments, we use a classifier free-guidance scale of $\alpha=15.0$ and $\alpha=7.5$; for composition experiments, we use $\alpha=7.5$ and $\beta=1.0$. For quantitative comparison, we fine-tuned the model for 500 steps. However, this may be sub-optimal depending on the subject and prompt complexity.

\section{User-Study Details}
In the user study, we asked 30 individuals to rate prompt alignment and personalization performances of four methods, including $P+$~\cite{PPLUS}, NeTI~\cite{NeTI}, TI~\cite{TI}+DB~\cite{DB}, and our method. Our test set includes six different subjects and ten prompts. We generated eight samples for each prompt and subject using the four methods. Then, we randomly picked a single photo and asked the participants to count the number of different prompt elements that appear in the generated image. We asked the users to rate the similarity between the main subject in the generated image and the sample. Then, we randomly divided the questions into three forms and shuffled them between the participants. Sample questions appear in~\cref{fig:user_study_sample_questions}.

\section{Over-saturation and mode-collapse in SDS}

The main paper uses prompt-aligned score sampling to guide the model towards the target prompt $y$. We found this to be more effective than using SDS~\cite{SDS} or improved versions of it like NFSD~\cite{NFSD}. In particular, SDS and NFSD produce over-saturated or less diverse results. We provide qualitative examples in~\cref{fig:sds_vs_ours}, and quantitative comparison appears in the main paper.

\section{Multi-subject Personalization}
\input{sup_figures/art_figure/fig}
\input{sup_figures/art_ablation/fig}
\input{sup_figures/sds_vs_ours/fig}


\paragraph{Multi-subject composition:} For multi-subject personalization, we use two placeholder $V_1$ and $V_2$ to represent the subject $S_1$ and $S_2$. We use $y_P$ = "A photo of [$V_i$]" as our personalization prompt. We use a descriptive prompt describing the desired scene for the target clean prompt. For example, "A 19th century portrait of a [$C_1$] and [$C_2$]", where $C_1$ and $C_2$ represent the class name of $S_1$ and $S_2$, respectively. We provide additional results in~\cref{fig:additional_composition}.

\paragraph{Art-inspired composition:} For Art-inspired composition, we use "A photo of [$V_1$]" to describe the main subject, while "An oil painting of [$V_2$]" is used for the artistic image. The clean prompt used is "An oil painting of [class name]," where "[class name]" is the subject class (e.g., a cat or a toy). Furthermore, adding a description to the clean prompt improves alignment, for example, "An oil painting of a cat sitting on a rock" for the" Wanderer above the Sea of Fog" artwork by Caspar David Friedrich. Finally, at test time, we use the target prompt "An oil painting of [$V_1$] inspired by [$V_2$] painting" or a similar variant, with possibly an additional description of the desired scene. Results appear in~\cref{fig:art_fig}. We further show that joint training is insufficient for this task, nor is pre-training on $S$ prompting the artwork or artist name. Both cases produce miss-aligned results (see~\cref{fig:art_ablation}).

\section{Over-fitting in Personalization Methods}
\input{figures/method_motivation/fig}
Long fine-tuning on a small image set could cause the model to overfit the target subject. As argued in the main paper, the model predictions always steer the backward denoising process towards one of the training images, regardless of any conditional prompt. In~\cref{fig:methodvisx0hat}, we visualize the model prediction by analyzing its estimate of $x_0$, the real-sample image. This estimate can be obtained from the forward denoising process via $\hat{x}_0$ equation, which is provided below for convenience:
\begin{equation}
   \hat{x}_0  = \frac{x_t - \sqrt{1-\bar{\alpha}_{t}}G_{\theta}(x_t,y) }{ \sqrt{\bar{\alpha}_{t}} }.
\end{equation} 

As can be seen from~\cref{fig:methodvisx0hat}, the pre-trained model (before personalization) steers the image towards a sketch-like image, where the estimate $\hat{x}_0$ has a white background, but the subject details are missing. Apply personalization without PALP overfits, where elements from the training images, like the background, are more dominant, and sketchiness fades away, suggesting miss-alignment with the prompt ``A sketch'' and over-fitting to the input image. Using PALP, the model prediction steers the backward-denoising process towards a sketch-like image, while staying personalized, where a cat like shape is restored.



\input{sup_figures/user_study_questions/fig}




\clearpage

\input{sup_figures/uncurated_faces/fig}

\input{sup_figures/LDM_Large/fig1}
\input{sup_figures/LDM_Large/fig2}

\input{sup_figures/qualitative_comp_additional/fig}

\input{sup_figures/faces_full/girl_fig}

\input{sup_figures/faces_full/guy_fig}


